StyleTTS: A Style-Based Generative Model for Natural and Diverse Text-to-Speech Synthesis

Text-to-Speech (TTS) has recently seen great progress in synthesizing high-quality speech owing to the rapid development of parallel TTS systems, but producing speech with naturalistic prosodic variations, speaking styles and emotional tones remains challenging. Moreover, since duration and speech are generated separately, parallel TTS models still have problems finding the best monotonic alignments that are crucial for naturalistic speech synthesis. Here, we propose StyleTTS, a style-based generative model for parallel TTS that can synthesize diverse speech with natural prosody from a reference speech utterance. With novel Transferable Monotonic Aligner (TMA) and duration-invariant data augmentation schemes, our method significantly outperforms state-of-the-art models on both single and multi-speaker datasets in subjective tests of speech naturalness and speaker similarity. Through self-supervised learning of the speaking styles, our model can synthesize speech with the same prosodic and emotional tone as any given reference speech without the need for explicitly labeling these categories.

==> cache.tex <==
%auto-ignore

\begin{table}[!htbp]
\caption{Comparison of evaluated MOS with 95\% confidence intervals (CI) on the LJ Speech dataset.}
\label{tab:1}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcr}
\toprule
Model & MOS-N (CI) \\ 
\midrule
Ground Truth              & 4.32 ($\pm$ 0.04)\\
Tacotron 2 + HiFi-GAN     & 3.01 ($\pm$ 0.06)\\
FastSpeech 2 + HiFi-GAN   & 2.97 ($\pm$ 0.06)\\
VITS                      & 3.78 ($\pm$ 0.06)\\
StyleTTS + HiFi-GAN    &\textbf{4.01} ($\pm$ \textbf{0.05})\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}




\begin{table}[!htbp]
\caption{Comparison of evaluated MOS with 95\% confidence intervals (CI) on the LibriTTS dataset. }
\label{tab:2}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
% \resizebox{\columnwidth}{!}
{%
\begin{tabular}{lccr}
\toprule
Model & MOS-N (CI) & MOS-S (CI) \\ 
\midrule
Ground Truth              & 4.35 ($\pm$ 0.04) & 3.90 ($\pm$ 0.07)\\
FastSpeech 2 + HiFi-GAN   & 3.00 ($\pm$ 0.06)  & 3.51 ($\pm$ 0.07)\\
StyleSpeech + HiFi-GAN    & 1.94 ($\pm$ 0.07) & 2.24 ($\pm$ 0.08)\\
VITS                      & 3.62 ($\pm$ 0.06) & 3.70 ($\pm$ 0.07)\\
StyleTTS + HiFi-GAN       & \textbf{4.03} ($\pm$ \textbf{0.05}) & \textbf{3.79} ($\pm$ \textbf{0.07})\\
\bottomrule
\end{tabular}}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


\begin{table}[!htbp]
\caption{Comparison of evaluated MOS with 95\% confidence intervals (CI) on the VCTK dataset for unseen speaker adaptation. }
\label{tab:3}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
% \resizebox{\columnwidth}{!}
{%
\begin{tabular}{lccr}
\toprule
Model & MOS-N (CI) & MOS-S (CI) \\ 
\midrule
Ground Truth              & 4.39 ($\pm$0.05) & 4.28 ($\pm$0.06)\\
StyleSpeech + HiFi-GAN    & 2.13 ($\pm$0.06) & 2.43 ($\pm$0.07)\\
StyleTTS + HiFi-GAN       & \textbf{3.55} ($\pm$\textbf{0.06}) & \textbf{3.57} ($\pm$\textbf{0.07})\\
\bottomrule
\end{tabular}}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}





\begin{table*}[!htbp]
\caption{Robustness evaluation on the LJSpeech and LibriTTS dataset. Word error rates (\%) are reported for different lengths of text (L).}
\label{tab:5}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccr}
\toprule
\multirow{2}{*}{Model} &  \multicolumn{4}{c}{WER ($\downarrow$)} \\ 
& $L \textless 10$ & $10 \textless L \textless 50$ & $50 \textless L \textless 100$ & $L \textgreater 100$ \\ 
\midrule
& \multicolumn{4}{c}{{\textit{Single-speaker models (on LJSpeech)}}} \\
Tacotron 2 + + HiFi-GAN & 17.22 & 12.61 & 16.95 & 46.33 \\
FastSpeech 2 + HiFi-GAN & 15.37 & 11.02 & 14.42 & 23.04 \\
VITS                    & 14.35 & 10.69 & 12.59 & 32.39 \\  
StyleTTS + HiFi-GAN     & \textbf{9.42}  & \textbf{7.44}  & \textbf{11.97} & \textbf{22.24} \\
\midrule
\midrule
& \multicolumn{4}{c}{{\textit{Multi-speaker models (on LibriTTS)}}} \\
FastSpeech 2 + HiFi-GAN  & \textbf{12.73} & 8.90  & 17.20 & 17.48 \\
StyleSpeech + + HiFi-GAN & 69.14 & 38.04 & 24.34 & 30.53\\
VITS                     & 20.97 & 15.67 & 20.95 & 21.05\\  
StyleTTS + HiFi-GAN      & 17.35 & \textbf{8.26} &  \textbf{14.58} & \textbf{15.83} \\

\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}



\begin{table}[!htbp]
\caption{Real time factor (RTF) in second. }
\label{tab:6}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcr}
\toprule
Model & RTF (s) \\ 
\midrule
Tacotron 2 + HiFi-GAN     &  0.0868\\
FastSpeech 2 + HiFi-GAN   &  \textbf{0.0095}\\
StyleSpeech 2 + HiFi-GAN  &  0.0337\\
VITS                      &  0.0428\\
StyleTTS + HiFi-GAN       &  0.0388\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}




\begin{table*}[!htbp]
\caption{Comparison of Pearson correlation coefficients of acoustic features associated with emotions between reference and synthesized speech in multi-speaker experiments. Fastspeech 2 and VITS employ the X-vector as the reference.}
\label{tab:7}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
% \begin{tabular}{lccccccccr}
\begin{tabular}{lcccccccr}
\toprule
Model & \makecell{Pitch \\mean} & \makecell{Pitch \\standard \\deviation} & \makecell{Energy \\mean} & \makecell{Energy \\standard \\deviation} & \makecell{Harmonics-\\to-noise \\ratio}  & \makecell{Speaking \\ rate} 
& Shimmer & Jitter \\
\midrule
FastSpeech 2    &0.95 &0.43 &0.23 & 0.51 & 0.81 
& \textbf{0.68} 
&0.81 &0.58\\
StyleSpeech     &0.68 &0.47 &0.22 &0.38 & 0.64 
& 0.23 
& 0.69 & 0.34 \\
VITS                      &0.97  &0.32 &0.14 &0.5 &0.84 
& 0.6 
&0.81 & 0.54\\
StyleTTS     &\textbf{0.99}  &\textbf{0.51} &\textbf{0.91} & \textbf{0.52}&\textbf{0.9} 
& 0.23 
&\textbf{0.87} & \textbf{0.65}\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}




\begin{table}[!htbp]
\caption{Style encoder and discriminator architectures. $T$ represents the input length of the mel-spectrogram, and $D$ is the output dimension. For style encoder, $D=128$. For discriminator, $D = 1$. }
\label{tab:9}

\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cccc}
\hline
Layer    & Pooling      & Norm & Output Shape \\ \hline

Mel x                     & -                           & -                        & 1$\times$80$\times T$                           \\ \hline
Conv 1$\times$1                  & -                           & -                        & 64$\times$80$\times T$                          \\
ResBlk                    & Dilated Conv                & -                        & 128$\times$40$\times T/2   $                    \\
ResBlk                    & Dilated Conv                & -                        & 256$\times$20$\times T/4$                       \\
ResBlk                    & Dilated Conv                & -                        & 512$\times$10$\times T/8$                       \\
ResBlk                    & Dilated Conv                & -                        & 512$\times$5$\times T/16 $                      \\ \hline
LReLU                     & -                           & -                        & 512$\times$5$\times T/16$                       \\
Conv 5$\times$5                  & -                           & -                        & 512$\times$1$\times T/80 $                      \\
LReLU                     & -                           & -                        & 512$\times$1$\times T/80$                       \\ \hline
-                         & AdaAvg                      & -                        & 512$\times$1                            \\
Linear                    & -                           & -                        & $D \times$1                            \\ \hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}




% \begin{wrapfigure}{r}{0.5\textwidth}
% \centering
% \includegraphics[width=0.48\textwidth]{figure/figure3.pdf}
% \caption{Spectrograms of example reference audios and their corresponding generated speech reading ``How much variation is there? Let's find it out." from the single-speaker model trained on LJSpeech. The estimated pitch contour is shown as white dots. \textbf{Left top}: Reference audio of a question, ``Did England let nature take her course?". Note the pitch is mostly going up at the end of each word. \textbf{Left bottom}: Synthesized speech. The same pattern of pitch rising at the end of the words is present. \textbf{Right top}: Reference audio of surprised speech saying ``It's true! I am shocked! My dreams!". Note the pitch goes up first and then down for each word. \textbf{Right bottom}: Synthesized speech with the same pattern of the pitch going up and down for most of the words.}
% \label{fig:3}
% \end{wrapfigure}

==> related_work.tex <==
%auto-ignore

\textbf{Text-to-Speech. } Traditionally, neural TTS models, including WaveNet \cite{oord2016wavenet}, SampleRNN \cite{mehri2016samplernn}, Deep-Voice 1, 2, 3 \cite{arik2017deep, gibiansky2017deep, ping2018deep}, Char2Wav \cite{sotelo2017char2wav}, and Tacorton 1/2 \cite{wang2017tacotron, shen2018natural}, are autoregressive speech generators. This results in slow inference and degradation in the quality of speech with long text. Recently, several works such as Parallel-Wavenet \cite{oord2018parallel}, FastSpeech 1/2 \cite{ren2019fastspeech, ren2021fastspeech}, WaveGlow \cite {prenger2019waveglow}, Glow-TTS \cite{kim2020glow} and VITS \cite{kim2021conditional} have proposed non-parallel TTS systems to address such issues in autoregressive models. Moreover, since phoneme duration is predicted independent of output speech, these models allow full control of the speed of synthesized speech. Models such as FastSpeech 2 \cite{ren2021fastspeech} and FastPicth \cite{lancucki2021fastpitch} also predict pitch and energy in addition to the phoneme duration and hence gain more control of the pitch and  energy of the synthesized speech.  

\textbf{Style Modulation. } Style-based models in the field of computer vision usually integrate conditional information (style) using conditional normalization such as adaptive instance normalization (AdaIN) \cite{huang2017arbitrary} and conditional batch normalization \cite{VriesSMLPC17}. AdaIN, in particular, has been been used for many applications such as improving image quality in adversarial generative network (GAN) models \cite{karras2019style, karras2020analyzing, karras2021alias}, neural style transfer \cite{huang2018multimodal, liu2019few, choi2020stargan} and image editing \cite{lee2020maskgan, zhu2020sean}. AdaIN predicts the gain and bias from an input style vector in an InstanecNorm \cite{ulyanov2016instance} module and is thus adaptive based on the input style vectors. 

\textbf{Stylizations in Text-to-Speech. } Previous works in stylizations of speech are mainly based on Tacotron \cite{wang2017tacotron}, an autoregressive TTS model that generates speech mel-spectrogram frame by frame. These models \cite{skerry2018towards, wang2018style, sun2020fully, liu2021expressive} learn a prosody encoder that extracts a style vector from reference, which is then either concatenated or summed frame-wise with the text encoder output. StyleSpeech \cite{min2021meta}, on the other hand, is a parallel TTS model that uses adaptive layer normalization (AdaLN) for zero-shot speaker adaptation. Unlike AdaIN, AdaLN applies the predicted gain and bias in a LayerNorm \cite{ba2016layer} module instead of an InstanceNorm module. 


